Stability-Preserving, Time-Efficient Mechanisms for School Choice in Two Rounds

We address the following dynamic version of the school choice question: a city, named City, admits students in two temporally-separated rounds, denoted $\mathcal{R}_1$ and $\mathcal{R}_2$. In round $\mathcal{R}_1$, the capacity of each school is fixed and mechanism $\mathcal{M}_1$ finds a student optimal stable matching. In round $\mathcal{R}_2$, certain parameters change, e.g., new students move into the City or the City is happy to allocate extra seats to specific schools. We study a number of Settings of this kind and give polynomial time algorithms for obtaining a stable matching for the new situations. It is well established that switching the school of a student midway, unsynchronized with her classmates, can cause traumatic effects. This fact guides us to two types of results, the first simply disallows any re-allocations in round $\mathcal{R}_2$, and the second asks for a stable matching that minimizes the number of re-allocations. For the latter, we prove that the stable matchings which minimize the number of re-allocations form a sublattice of the lattice of stable matchings. Observations about incentive compatibility are woven into these results. We also give a third type of results, namely proofs of NP-hardness for a mechanism for round $\mathcal{R}_2$ under certain settings.

==> S_3_4.tex <==
\subsection{Setting B1 and B2}


We prove Theorem $\ref{thm:S3}, \ref{thm:S4}$ by providing polynomial time reductions from Setting B1, and Setting B2 to the case of unit capacities.\\

\noindent\textbf{Reduction from Setting B1 to Unit-Capacity}:\\
Let $I$ be the stable matching instance defined by Setting $B1$, where $I$ is defined over $(S, H \union H', c)$ with preference lists $l(s_i) \ \forall s_i \in S \cup N, \textnormal{ and } l(h_j) \ \forall h_j \in H$. To reduce this to an instance, $I'$, of unit capacity defined over $(A, B \union B', E')$ with preference lists $l'(a_i) \ \forall a_i \in A$ and $l'(b_j) \ \forall b_j \in B \union B' $ let:
\begin{itemize}
	\item $A = S$

	\item $B = \Union_{h \in H}\{h^{(1)},..., h^{c(h)}\}$, i.e. for each school create a vertex for each available seat.

	\item $E$ =  edge between $s_i, h^{j}_{i}$, \textbf{iff}, $s_i$ comes before $\emptyset$ on $l(h_{j})$ and $h_j$ comes before $\emptyset$ in $l(s_i)$

	\item $M = \phi(M^*)$, where $M^*$ is a Student-Optimal Stable Matching of $I$ computed in $\cR_1$, and $\phi$ is defined below.

	\item $B' =  \Union_{h \in H'}\{h^{(1)},..., h^{c(h)}\}$, creating seats for the new schools


	\item $E' = E \union \{(s_i, h^{i}_j)| h_j \in H' \textnormal{ and } s_i, h_j \textnormal{ come before } \emptyset \textnormal{ on each others preference lists} \}$

	
	\item $\forall s_i \in S$, $l'(s_i)$ is obtained by replacing each school $h_j$, in $l(s_i)$ by $[h_{j}^{1},\hdots, h_{j}^{c(h_j)}]$

	\item $\forall h_j \in H\cup H'$, and $i \leq c(h_j),\ l'(h_{j}^{i}) = l(h_j)$






\end{itemize}

\begin{lemma}
There exists a bijection, $\phi$, between the sets of stable matchings in $I$ and $I'$
\end{lemma}

\begin{proof}

	Let $M$ be a stable matching for $I$, we will construct an equivalent stable matching $\phi(M)$ for $I'$. 
	If $s_i$ is matched to $h_j$ in $M$, and $s_i$ is ranked $k$ among the students matched to $h_j$, then $s_i$ would be matched to $h_{j}^{k}$ in $\phi(M)$.\\
	To argue stability let there be a blocking pair $(s_i, h_{j}^{k})$ with respect to $\phi(M)$, then $s_i$ must prefer $h_{j}^{k}$ to its current partner, say $h_{l}^{k'}$. There are three cases to consider: $h_{l}^{k'}$ = $\emptyset$, $l \neq j$, or $l = j$. The first two cases would result in a blocking pair between $(s_i, h_j)$ in $M$ which is a contradiction.
	Finally for the case when $l=j$, by construction of preference lists, if $k' < k$ then this would contradict $(s_i, h_{j}^{k})$ being a blocking pair, and if $k' > k$ then this would contradict $s_i$ being ranked $k'$ among students matched to $h_j$ in $M$.\\	
	For the other direction let $M'$ be a stable matching in $I'$, the inverse of $\phi$ can be computed by sending $s_i$ to $h_j$, if $s_i$ is matched to $h_{j}^{k}$ in $M'$. The stability of $\phi^{-1}(M')$ follows since each school $h_{j}$ has the same preference lists as $h_{j}^{i}$ for $i \in [1, \hdots ,c(h_j)]$\\\\ 

\end{proof}

\noindent \textbf{Reduction from Setting B2 to Unit-Capacity:}\\
Let $I$ be the stable matching instance defined by Setting $B2$, where $I$ is defined over $(S \union N, H, c)$ with preference lists $l(s_i) \ \forall s_i \in S \cup N, \textnormal{ and } l(h_j) \ \forall h_j \in H$. To reduce this to an instance, $I'$, of unit capacity defined over $(A, B \union B', E')$ with preference lists $l'(a_i) \ \forall a_i \in A$ and $l'(b_j) \ \forall b_j \in B \union B' $ let:
\begin{itemize}

	\item $A = \Union_{h \in H}\{h^{(1)},..., h^{c(h)}\}$, i.e. for each school create a vertex for each available seat.



	\item B = $S$

	\item $E$  =  edge between $s_i, h^{j}_{i}$, \textbf{iff}, $s_i$ comes before $\emptyset$ on $l(h_j)$ and $h_j$ comes before $\emptyset$ in $l(s_i)$



	\item $M = \phi(M^*)$, where $M^*$ is a Student-Optimal Stable Matching of $I$ computed in $\cR_1$, and $\phi$ is defined below.

	\item $B' = N$

	\item $E' = E \union \{(s_i, h_{j}^{i}) | s_i \in N$ and $s_i, h_j$ come before $\emptyset$ on each others preference lists    $ \} $


	\item $\forall s_i \in B \union B'$, $l'(s_i)$ is obtained by replacing each school $h_j$, in $l(s_i)$ by $[h_{j}^{1},\hdots, h_{j}^{c(h_j)}]$

	\item $\forall h_j \in A$, and $i \leq c(h_j), \ l'(h_{j}^{i}) = l(h_j)$

\end{itemize}
	
The bijection, $\phi$, between $I$ and $I'$, is identical from the previous reduction.\\\\



\begin{proof} {\em of Theorem \ref{thm:S3} :}\\
	We can apply Reduction $1$ to an instance of Setting $B1$, in polynomial time. This reduces the problem of finding a minimum stable re-allocaion to the unit-capacity setting. Applying Theorem $\ref{sec:new_participants_theorem}$, on the reduced instance we get a minimum stable re-allocation in the unit capacity setting. We can then apply the inverse map, $\phi^{-1}$, from the reduction to get a stable matching over students and schools that is a minimum stable re-allocation.\\

\end{proof}


\begin{proof}{\em of Theorem \ref{thm:S4}: }\\
	The proof is symmetric after applying Reduction $2$ to an instance of Setting $B2$.
\end{proof}


==> impossibility.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\section{Impossibility Results}
\label{sec.impossibility}


In this section, we will prove the two impossibility results we described in Section \ref{sec:S3}. For this purpose, we will first need to enhance Example \ref{ex.1} to the much more sophisticated and carefully designed Example \ref{ex:2}.


\begin{example}
\label{ex:2}
	Assume there are 4 students $A,B,C,D$ and 3 schools 1,2,3. The preferences for $A,B,C,D$ are $(1,2,3), (2,1,3), (2,3,1), (2,3,1)$, respectively. The preferences for $1,2,3$ are $(B,A,C,D)$, $(A,C,B,D)$, $(C,B,A,D)$, respectively. In $\cR_1$, each school has 1 seat. 
	The only stable matching when all students come in round $\cR_1$ is $(1B, 2A, 3C)$.	%Hence, choosing neither of the two possible matchings results in a DSIC mechanism.
\end{example} 

\begin{theorem}
	\label{thm:impossible1}
There is no pair of non-oblivious, stability-preserving, DSIC mechanisms $(\cM_1, \cM_2)$ for Setting III.	
\end{theorem}

\begin{proof}
Assume that $(\cM_1, \cM_2)$ is a pair of non-oblivious, stability-preserving, DSIC mechanisms for Setting III. We will run them on three instances derived from Example \ref{ex:2}. In all three instances, the set of students and schools, $S$ and $H$, are the same as in Example \ref{ex:2}; what differs is the partition of $S$ into $S_1, S_2$.


\begin{itemize}
	\item {\bf $I_1$:} \hspace*{.4cm} $S_1 = \{A,B,C,D\}$ and $S_2 = \emptyset$.
	\item {\bf $I_2$:} \hspace*{.4cm} $S_1 = \{A,B,D\}$ and $S_2 = \{C\}$.
	\item {\bf $I_3$:} \hspace*{.4cm} $S_1 = \{A,D\}$ and $S_2 = \{B,C\}$.
\end{itemize}

As stated in Example \ref{ex:2}, in $I_1$, $\cM_1$ is forced to pick the unique stable matching $(1B, 2A, 3C)$, in which $C$ is matched to school 3. In $I_2$, mechanism $\cM_1$ can choose one of two possible stable matchings, $(1B, 2A, 3D)$ or $(1A, 2B, 3D)$. Let us consider both possibilities.
		\begin{enumerate}
		\item $(1A, 2B, 3D)$ is chosen. When $C$ participates in round $\cR_2$, she has to be assigned to school 2 by $\cM_2$ in order to preserve stability. Since she prefers school 2 to school 3, she has incentive to cheat.
		
		\item $(1B, 2A, 3D)$ is chosen. In this matching, $B$ is matched to school 1.
		Now, we consider instance $I_3$ in which $\cM_1$ is forced to pick the unique stable matching $(1A, 2D)$. When $B$ and $C$ participate in round $\cR_2$, mechanism $\cM_2$ will have to match $B$ to school 2 so that stability is preserved. Since $B$ prefers school 2 to school 1, she has incentive to cheat.
	   \end{enumerate}
	   
	   Therefore, for each of the choices, the pair of mechanisms $(\cM_1, \cM_2)$ fails to be DSIC on at least one of the instances. The contradiction completes the proof.

\end{proof}

\begin{remark}
Observe that in the proof given above, $B$ was able to cheat when another student, namely $C$, was also cheating. In contrast, Theorem \ref{thm:S3} gives a pair of mechanisms under which $B$ would not be able to cheat if no other student were cheating.   
\end{remark}

\begin{theorem}
	\label{thm:impossible2}
There is no pair of oblivious, stability-preserving, ICNE mechanisms $(\cM_1, \cM_2)$ that ensure that residents of the City can't gain by opting to participate in round $\cR_2$ and not in round $\cR_1$.
\end{theorem}

\begin{proof}
Assume that $(\cM_1, \cM_2)$ is a pair of oblivious, stability-preserving, ICNE mechanisms for Setting III. We will run them on four instances derived from Example \ref{ex:2}. In the first two instances, the set of students and schools, $S$ and $H$, are the same as in Example \ref{ex:2}, and in the last two, $S = \{A,B,D\}$ and $H$ is the same as in Example \ref{ex:2}. The partition of $S$ into $S_1, S_2$ is as follows:

\begin{itemize}
	\item {\bf $I_1$:} \hspace*{.4cm} $S_1 = \{A,B,C,D\}$ and $S_2 = \emptyset$.
	\item {\bf $I_2$:} \hspace*{.4cm} $S_1 = \{A,B,D\}$ and $S_2 = \{C\}$.
	\item {\bf $I_3$:} \hspace*{.4cm} $S_1 = \{A,B,D\}$ and $S_2 = \emptyset$.
	\item {\bf $I_4$:} \hspace*{.4cm} $S_1 = \{A,D\}$ and $S_2 = \{B\}$.
\end{itemize}
Since the mechanisms are oblivious, in each run, they ``know'' the preference lists of students participating in that round only. 

As stated in Example \ref{ex:2}, in $I_1$, $\cM_1$ is forced to pick the unique stable matching $(1B, 2A, 3C)$, in which $C$ is matched to school 3. In $I_2$, mechanism $\cM_1$ can choose one of two possible stable matchings, $(1B, 2A, 3D)$ or $(1A, 2B, 3D)$. Let us consider both possibilities.
		\begin{enumerate}
		\item $(1A, 2B, 3D)$ is chosen. When $C$ participates in round $\cR_2$, she has to be assigned to school 2 by $\cM_2$ in order to preserve stability. Since she prefers school 2 to school 3, she has incentive to cheat even when the rest are telling the truth.
		
		\item $(1B, 2A, 3D)$ is chosen. We now consider instance $I_3$. Since $\cM_1$ is oblivious, it cannot distinguish between $I_2$ and $I_3$, and it therefore chooses the stable matching $(1A, 2B, 3D)$ for $I_3$ as well. Note that $B$ is assigned to school 2 in this matching.
		
		Finally, we consider instance $I_4$ in which $\cM_1$ picks the unique stable matching $(1A, 2D)$. When $B$ participates in round $\cR_2$, mechanism $\cM_2$ will have to match her to school 2 so that stability is preserved. Since $B$ prefers school 2 to school 1, she has incentive to cheat even when the rest are telling the truth.
	   \end{enumerate}
	   
	   Therefore, for each of the choices, the pair of mechanisms $(\cM_1, \cM_2)$ fails to be ICNE on at least one of the instances. The contradiction completes the proof.
\end{proof}

From a mathematical viewpoint, perhaps the most interesting aspect of this pair of proofs is the subtle, though key, contrast that arises because of the difference in the information revealed to the mechanisms. 






==> s3.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Setting III}
\label{sec:mS3}


Theorems \ref{thm:impossible1} and \ref{thm:impossible2} leave the possibility of obtaining a pair of non-oblivious, stability-preserving, ICNE mechanisms for Setting III, and this is what we present next. Additionally, both our mechanisms run in polynomial time. 


The mechanisms $\cM_1$ and $\cM_2$ are given in Figures \ref{alg:S3M1} and \ref{alg:S3M2} respectively. $\cM_1$ first computes the student-optimal matching for all students in $S$. Then all students in $(S-S_1)$ are removed from the matching. In general, this will create under-filled schools and hence type 2 blocking pairs. While there exists a blocking pair of type 2, involving a school $h_j$, say, the student $s_i = \BStP(h_j)$ is reassigned to $h_j$. This cannot create a type 1 blocking pair, as proven in Lemma~\ref{lem:m1stable}. However, it decreases the extent to which $h_j$ is under-filled, but increases the extent to which school $h_k$ is under-filled, where $h_k$ is the school to which $s_i$ was previously assigned. We show below that this process must terminate in a stable matching in polynomial time.

\begin{figure}
	\begin{wbox}
		\textsc{$\cM_1$}$(S,S_1,H,c)$: \\
		\textbf{Input:} Sets $S$ of students, $H$ of schools, and $S_1 \subseteq S$ of students participating in round $\cR_1$.  \\
		\textbf{Output:} Stable matching $M$ from $S_1$ to $H \union \{\emptyset\}$. \\ 
		\begin{enumerate}
		\item $M \leftarrow$ Student-optimal stable matching from $S$ to $H \union \{\emptyset\}$ under school capacities $c$.  \\
		%$S_0 \leftarrow$ students in $S$ that are matched to $\emptyset$ in $M_0$.  \\\\
		\item Remove all students of $(S - S_1)$ from $M$. \\
		%Initialize $R$ to an empty set. \\\\  
		\item While $\exists$ school $h_j$ which participates in a type 2 blocking pair: \\
		\begin{enumerate}
		\item Let $s_i = \BStP(h_j)$. \\
		\item $M \leftarrow M \union \{(s_i, h_j)\}$. \\
		\end{enumerate}
		\item Return $M$.
		\end{enumerate}
	\end{wbox}
	\caption{Mechanism for round $\cR_1$ in Setting III}
	\label{alg:S3M1} 
\end{figure} 


\begin{figure}
	\begin{wbox}
		$\cM_2(M, S_2, N,L)$: \\
		\textbf{Input:} Stable matching $M$ and sets $S_2$, $N$, $L$.  \\
		\textbf{Output:} Stable, IC, $Min_{S_2 \cup N} Max_L$ extension of $M$. \\ 
		\begin{enumerate}
			\item $\forall s_i \in S_M: M'(s_i) \leftarrow M(s_i).$ \\ 
		    \item $S_2' \lla \{s_i \in S_2 ~|~   \PgSch(s_i) \ \mbox{is non-empty} \}$. \\
			\item $ \forall s_i \in S_2' :  M'(s_i) \leftarrow \text{Best school for} \ s_i \ \mbox{in} \ \PgSch(s_i). $ \\
			\item $\forall h_j \in H: \ \Barr1 (h_j) \lla \ \BStP (h_j; S_M)$. \\	
		    \item $\forall h_j \in H: \ \Barr2 (h_j) \lla \ \mbox{Best student for} \ h_j \ \mbox{in} \ (N - N')  \cup (S_2 - S_2')$. \\
			\item $\forall h_j \in H: \ \Barr3 (h_j) \lla \BStP(h_j; S_2). $ \\		
			\item $\forall h_j \in H: \ \Barr (h_j) \lla \ \mbox{Best student for} \ h_j \ \mbox{in} \ \{\Barr1(h_j), \Barr2(h_j), \Barr3(h_j) \}$. \\	
			\item $N' \lla \{s_i \in N ~|~   \PgSch(s_i) \ \mbox{is non-empty} \}$. \\
		    \item $L' \lla \{ s_i \in L  ~|~  \exists h_j \ \mbox{s.t. $s_i$ appears before $\Barr (h_j)$ in $l(h_j)$}$, \\
			\hspace*{2.4cm} $\mbox{and $h_j$ appears before $\emptyset$ in $l(s_i)$} \}$. \\
			\item $\forall s_i \in (N' \cup L'): \ \FSch(s_i) \lla \{ h_j ~|~  s_i \ \mbox{appears before} \ 
			\Barr(h_j) \ \mbox{in} \ l(h_j) \}$. \\
			\item $\forall s_i \in (N' \cup L'): \ M'(s_i) \lla \ \mbox{Best school for} \ s_i \ \mbox{in} \ \FSch(s_i)$. \\
			\item $\forall s_i \in (N - N') \cup (S_2 - S_2') : M'(s_i) \leftarrow \emptyset. $ \\
			\item $\forall s_i \in (L - L'): M'(s_i) \leftarrow \emptyset$.  \\
			\item Return $M'$. 
		\end{enumerate}
	\end{wbox}
	\caption{Mechanism for round $\cR_2$ in Setting III}
	\label{alg:S3M2} 
\end{figure}



\begin{lemma}
	\label{lem:m1time}
	Step 3 in mechanism $\cM_1$, given in Figure~\ref{alg:S3M1}, runs in polynomial time.
\end{lemma} 
\begin{proof}
	Each time a reassignment is done, the school of the reassigned student improves. Therefore, at most $nm$ reassignments can be done. 
\end{proof}
 


\begin{lemma}
	\label{lem:m1stable}
	The matching $M$ returned by $\cM_1$ is stable.
\end{lemma}
\begin{proof}
	Clearly, the matching obtained in Step 1 is stable. 
	Step 2 introduces only blocking pairs of type 2. 
	Hence, at the beginning of Step 3, where the reassignments are made, only blocking pairs of type 2 exist. 
	A reassignment for school $h_j$ matches $h_j$ to $s_i = \BStP(h_j)$. Hence, after the reassignment,  $s_i$ becomes $\LPSt(h_j)$, and the new $\BStP(h_j)$ if it exists, must appear after $s_i$ in the preference list of $h_j$.
	By Lemma~\ref{lem:blocking}, no blocking pairs of type 1 are created.  
	Step 3 terminates when there are no more blocking pairs of type 2; by Lemma~\ref{lem:m1time}, this takes at most $nm$ iterations of Step 3. Hence, the matching output by $\cM_1$ is stable.
	\end{proof}

The second mechanism $\cM_2$ is similar to the one given in Figure~\ref{alg:S2,1}. However, the setting is much more complex, making it necessary to give new definitions for some of the terms, with two parameters instead of one. For each student $s_i \in S_M$, the definition of {\em set of schools preferred by $s_i$} remains the same as before and is denoted by $\PSch (s_i)$. For each school $h_j \in H$ and set of students $T$, define the {\em set of students from T that prefer $h_j$ over the school they are assigned to}, denoted $\PSt (h_j; T)$ to be $\{ s_i \in T ~|~  h_j \in \PSch (s_i)  \}$. Finally, define the {\em best student from T preferring $h_j$}, denoted $\BStP(h_j; T)$, to be the student from $T$ whom $h_j$ prefers the best in the set $\PSt(h_j; T)$. If $\PSt (h_j; T) = \emptyset$ then we will define $\BStP (h_j; T) = \emptyset$; in particular, this happens if $h_j$ is under-filled.



The main new difference from the mechanism of round $\cR_2$ in Setting II is the manner in which a student $s_i \in S_2'$ is assigned to a school. In particular, this is different from the way $s_i \in (N' \cup L')$ is assigned to a school. Indeed, if  $s_i \in S_2'$ were assigned a school in the same way as $s_i \in (N' \cup L')$, then she could end up getting a better school by gaming the round she participates in. Hence, this difference is critical to ensuring that the mechanism is ICNE.
  
By a similar argument to the one given in Section~\ref{sec:mS2}, we have the following lemma:

\begin{lemma}
	\label{lem:m2stable}
	The matching $M'$ returned by $\cM_2$ is stable.
\end{lemma}










==> unit_case.tex <==
\section{Mechanisms for Type B}
\subsection{Minimum Stable Re-allocations in the Unit Capacity Case}

Consider a stable matching instance over a bipartite graph  $ (A,B,E)$, where $A$ and $B$ are the sets of the bipartition. All members of $A$ (resp. B) have ordered preference lists over members in $B$ (resp. A). An edge between $a_i \in A$ and $b_j \in B$ indicates that $a_i$ and $b_j$ prefer being matched to each other over being matched to $\emptyset$.\\


In Round $\cR_1$ a stable matching, $M$, is found over $(A,B,E)$. $A_M \subseteq A$ represents the members of $A$ matched in round $\cR_1$, while $A_L = A - A_M$, represents the members who remain unmatched after round $\cR_1$. In $\cR_2$ a set of new participants $B'$ arrive. Let us denote the new graph as $G = (A, B \union B', E')$, and let $S_{G}$ represent the set of stable matchings over $G$.


\begin{definition} \textbf{(Minimum Stable Re-allocation of M)}: Is a stable matching $M'$ over $G$, where the number of members $a_i \in A_M$ such that $M(a_i) \neq M'(a_i)$ is minimized.
\end{definition}





A natural approach to finding a minimum stable re-allocation would be to apply Gale-Shapley on the updated instance $G$, but Example $\ref{ex:GS_bad_MSR}$ shows that this could require as many as $| A |$ possible re-allocations.


\begin{example}\label{ex:GS_bad_MSR}
Assume there are $n+1$ members in both sets $A$ and $B$. Let the preference lists be as follows:\\

\begin{table}[hbt!]
	\begin{tabular}{lllllllllllllll}
		\bm{$a_{1}:$} & $b_{n+1}$  & $b_{1}$ & $b_{2}$ & ....  &  $b_{n}$ & &  &  	\bm{$b_{1}:$} & $a_{1}$  & $a_{2}$ & $a_{3}$ & ....  &  $a_{n+1}$ &  \\

		\bm{$a_2:$} & $b_{1}$  & $b_{2}$ & $b_{3}$ & ....  &  $b_{n+1}$ & &  &       \bm{$b_2:$} & $a_{2}$  & $a_{3}$ & $a_{4}$ & ....  &  $a_{1}$ &  \\
		\bm{$a_3:$} & $b_{2}$  & $b_{3}$ & $b_{4}$ & ....  &  $b_{1}$ & & &         \bm{$b_3:$} & $a_{3}$  & $a_{4}$ & $a_{5}$ & ....  &  $b_{2}$ &  \\
		\vdots & \vdots & \vdots & \vdots & & \vdots  & & &	\vdots & \vdots & \vdots & \vdots & & \vdots   \\

		\bm{$a_{n}:$} & $b_{n-1}$  & $b_{n}$ & $b_{n+1}$ & ....  &  $b_{n-2}$ & & & 	\bm{$b_{n}:$} & $a_{n}$  & $a_{n+1}$ & $a_{1}$ & ....  &  $a_{n-1}$ &  \\
		\bm{$a_{n+1}:$} & $b_{n}$  & $b_{n+1}$ & $b_{1}$ & ....  &  $b_{n-1}$ & & & 	\bm{$b_{n+1}:$} & $a_{n+1}$  & $a_{1}$ & $a_{2}$ & ....  &  $a_{n}$ &  \\
	
	\end{tabular}
\end{table}


In Round $\cR_1$ all participants but $b_{n+1}$ are present. In Round $\cR_2$  $b_{n+1}$ arrives. The only stable matching, M, from $\cR_1$ would match each $a_i \rightarrow b_i$ and $a_{n+1}$ would remain unmatched. Assigning $a_{n+1}$ to $b_{n+1}$ would result in a stable matching requiring no re-allocations. However, running Gale-Shapley over all particpants would yield the matching where each $a_{i} \rightarrow b_{i-1}$, but this matching requires $n$ re-allocations.\\


\end{example}




\begin{lemma}\label{sec:new_participant_lemma}
Under the addition of new participants $B'$, each member of $A$ weakly improves in any minimum stable re-allocation of $M$.
\end{lemma}

\begin{proof}
	Let $M'$ be a minimum stable re-allocation of $M$, such that some students prefer their partner in $M$ to $M'$. Let $W$ denote these set of students. Consider $M^* = M \vee M'$, the matching where each $a_i$ chooses the partner it prefers between $M(a_i)$, $M'(a_i)$. We show that $M^*$ is a stable matching.\\
	Let $a_i \in W$, then $M^*$ only moves $a_i$ to its original partner in $M$. $M(a_i)$ must be matched to someone in $M'$, otherwise $(a_i, M(a_i))$ would form a blocking pair. Let $a_j$ be matched to $M(a_i)$ in $M'$, then $a_j$ must also be in $W$, since otherwise $(a_j, M(a_i))$ would form a blocking pair in $M$. Thus moving all the $a_i \in W$ back to their orignial schools still results in a valid matching.\\
To argue stability, let $(a_i, b_i), (a_j, b_j) \in M^*$, and $(a_i, b_j)$ be a blocking pair. Then $a_i$ is matched to $b_i$ or worse in both $M$ and $M'$, but $(a_j, b_j)$ must be in one of these matchings contradicting stability.\\
$M^*$ is a stable re-allocation of $M$ requiring $|W|$ fewer re-allocations than $M'$, a contradiction.\\
\end{proof}


Let $MSR$, denote the set of all minimum stable re-allocations of $M$ over $G$.

\begin{definition}  
$a_i$ is \textbf{moved} in $M' \in MSR$, if $M(a_i) \neq M'(a_i)$
\end{definition}



\begin{lemma}\label{sec:participants_fixed_lemma}
    All minimum stable re-allocations of $M$ over $G$ move the same members of $A$, $A_R$
\end{lemma}


\begin{proof}
We consider two cases, $a_i \in A_M$ and $a_i \in A_L$.
When $a_i \in A_L$, let $M'$ be any minimum stable re-allocation of $M$. By Rural Hospitals Theorem, the members of $A$ who are unmatched in $M'$ cannot be matched in any stable matching, and the members in $A_L$ who do get matched in $M'$ must be matched in all stable matchings over $G$. Thus, if $a_i \in A_L$ such that $M'(a_i) \neq \emptyset$ then $a_i$ must be moved in all $MSR$.

For the case when $a_i \in A_M$, let there be two $MSR$ $M', M''$, such that there exists $a_i$ where $M(a_i) = M'(a_i) \neq M''(a_i)$. Then the following sets include all possiblilities for $a_i$:
	\begin{itemize}
		\item $A_{1} = \{a_i \in A_M \ | \ M(a_i) = M'(a_i) \neq M''(a_i) \}$
		\item $A_{2}	= \{ a_i \in A_M \ | \ M(a_i) = M''(a_i) \neq M'(a_i) \}$
		\item $A_{3} = \{ a_i \in A_M \ | \ M(a_i) \neq M'(a_i) \textnormal{ and } M(a_i) \neq M''(a_i) \}$
		\item $A_{4} = \{a_i \in A_M \ | \ M(a_i) =  M'(a_i) = M''(a_i) \}$
	\end{itemize}

	Now if we consider the matching $M_L = M \wedge M'$(the partner they prefer less)  this will send all $a_i \in A_{1}, A_{2}, A_{4}$ to their original partners in $M$, since from Lemma $\ref{sec:new_participant_lemma}$ we have that each $a_i$ must weakly improve in any $MSR$. From Theorem $\ref{sec:stable-matching-lattice}$, $M_L$ is the meet of two stable matchings and hence a stable matching.\\
The number of re-allocations in $M'  = |A_{3}| + |A_{2}|$.\\
The number of re-allocations  in $M'' = |A_{3}| + |A_{1}|$.\\
The number of re-allocations in $M_L = |A_{3}|$.\\
By assumption $A_{1}$ is non-empty and thus $M_L$ requires fewer re-allocations than $M'$, a contradiction. Thus if $a_i$ is moved in one re-allocation it is moved in all re-allocations.\\
\end{proof}

\begin{corollary} \label{sec:same-B}
All minimum stable re-allocations move the same members of $B \union B'$, $B_R$. 
\end{corollary}

\begin{corollary}\label{sec:A_F-fixed}
All $a_i \in A - A_R$ have the same partner in all minimum stable re-allocations.
\end{corollary}

\noindent We denote these students $A_F$ and let $M_F$ represent the matching restricted to these students. Then for all $M' \in MSR$ and $a_i \in A_F, M_F(a_i) = M(a_i) = M'(a_i)$. Let $B_F$ represent the members of $B \union B'$ matched to $A_F$ in all $MSR$.\\

\noindent Consider the Graph $G' \subseteq G$, defined below:\\

\begin{itemize}

	\item $\forall b_j \in B_R, \ \Barr(b_j) = $ Most preferred $a_i \in A_F$ in $b_j$ preference list such that $(a_i, b_j) \subseteq E'$, and $a_i$ prefers $b_j$ to $M(a_i)$.
	
	\item $\forall a_i \in A_R, \ \Barr(a_i) = $ Most preferred $b_j \in B_F$ in $b_j$ preference list such that $(a_i, b_j) \subseteq E'$, and $b_j$ prefers $a_i$ to $M(b_j)$.

	\item $E'' = \{(a_i, b_j) \in E' \ | \ a_i \in A_R, b_j \in B_R,$ $b_j$ prefers $a_i$ to $\Barr(b_j)$, and $a_i$ prefers $b_j$ to $\Barr(a_i) \}$ 
	

	\item $G' = (A_R, B_R, E'')$
	
\end{itemize}


\begin{lemma}\label{sec:allowed-edges}
	Any edge $e \in E'$,  between $a_i \in A_R$ and $b_i \in B_R$ not in $E''$, cannot be in any minimum stable reallocation.
\end{lemma}



\begin{proof}
	Let $M'$ be a minimum stable re-allocation where such an edge $(a_i, b_j)$ exists. By construction $a_i$ must be to the right of $\Barr(b_j)$ on $b_j$'s preference list, or $b_j$ must be to the right of $\Barr(a_i)$ on $a_i$'s preference list.\\
    $\Barr(b_j) \in A_F$ and so its partner is fixed in all $MSR$ by Corollary $\ref{sec:A_F-fixed}$. $\Barr(b_j)$ prefers $b_j$ to its partner in $M$, and if $a_i$ is  to the right of $\Barr(b_j)$ on $l(b_j)$ then $(\Barr(b_j), b_j)$ forms a blocking pair in $M'$. Similarly if $b_j$ is to the right of $\Barr(a_i)$ on $l(a_i)$ then $(a_i, \Barr(a_i))$ would form a blocking pair in $M'$, either way a contradiction. 
	
	
\end{proof}



\noindent Let $S_{G'}$ denote the set of stable matchings over $G'$.

\begin{lemma}\label{sec:compose-lemma}
	$\forall \ M_{G'} \in S_{G'}, M'= M_{G'} \union M_F$ is a minimum stable re-allocation.
\end{lemma}

\begin{proof}
	We only need to show that $M'$ is stable. Let $(a_i, b_j)$ be a blocking pair to $M'$, then $a_i \in A_F$ and $b_j \in B_R$, or $a_i \in A_R$ and $b_j \in B _F$. Consider the case where $a_i \in A_F$ and $b_j \in B_R$, and let $M'(b_j) = a_j$. $b_j$ must prefer $a_i$ to its partner in $M'$. Then $a_i$ is ranked atleast as high as $\Barr(b_j)$ and $a_j$ comes after the Barrier on $b_j$'s preference list. Hence $(a_j, b_j) \not\in  E''$, a contradiction.
    A similar argument works for the case when $a_i \in A_R$ and $b_j \in B_F$.
\end{proof}


\begin{lemma} \label{sec:decompose-lemma}
	Any $M' \in MSR$ can be decomposed into $M_{G'} \union M_F$, where $M_{G'} \in S_{G'}$.

\end{lemma}


\begin{proof}
	By Corllary $\ref{sec:A_F-fixed}$, $M_F \subseteq M'$. By Corollary $\ref{sec:same-B}$, students in $A_R$ must be matched to students in $B_R$. Restricting $M'$ to students in $A_R$, there must be a stable matching over $(A_R, B_R, E')$. By Lemma $\ref{sec:allowed-edges}$, the only edges between $A_R$ and $B_R$ not included in $E''$ can never be part of any $MSR$. Hence $M'$ restricted to students in $A_R$ must be a stable matching over $(A_R, B_R, E'') = G'$. 

\end{proof}

\begin{lemma} 
	$(MSR, \succeq)$ defines a sub-lattice of $(S_{G}, \succeq)$.
\end{lemma}

\begin{proof}
Let $M_1, M_2 \in MSR$. Define $M_U = M_1 \vee M_2$, and $M_L = M_1 \wedge M_2$, where for each $a_i, \ M_U(a_i)$ is the partner it weakly prefers in $M_1(a_i), M_2(a_i)$ and $M_L(a_i)$ is the complement of $M_U(a_i)$.\\
By Lemma $\ref{sec:decompose-lemma}$, we can decompose $M_1$ as $M_{G'}^{1} \union M_F$, and $M_2$ as $M_{G'}^{2} \union M_F$ where $M_{G'}^{1}$ and $M_{G'}^{2} \in S_{G'}$. For $a_i \in A_F$, $M_1 \vee M_2 = M_1 \wedge M_2 = M_F$. 
For $a_i \in A_R$ since $M_{G'}^{1}, M_{G'}^{2} \in S_{G'}$ by Theorem $\ref{sec:stable-matching-lattice}$, $ \ M_{G'}^{1} \vee M_{G'}^{2}$ and $M_{G'}^{1} \wedge M_{G'}^{2}$ are also stable matchings in $S_{G'}$. Then from Lemma $\ref{sec:compose-lemma}$ $M_U = M_{G'}^{1} \vee M_{G'}^{2} \union M_F$ is a MSR, and $M_L = M_{G'}^{1} \wedge M_{G'}^{2} \union M_F$ is also MSR. Thus $M_L$ and $M_U$ are the meet and join of two minimum stable re-allocations. \\


\end{proof}

\noindent The lattice structure defined above, leads to the following definitions:


\begin{definition} \textbf{A-Optimal Minimum Stable Re-allocation:}\\
Each member $a_i \in A_R$ is matched to its best possible partner among all minimum stable re-allocations.\\
\end {definition}

\begin{definition} \textbf{A-Pessimal Minimum Stable Re-allocation:}\\
Each member $a_i \in A_R$ is matched to its worst possible partner among all minimum stable re-allocations\

\end{definition}


\begin{figure}[htbp]
	\begin{wbox}
		\textsc{Adding New B}$(M, A, B \cup B')$: \\
		\textbf{Input:} Stable matching $M$ and bipartite graph $G=(A, B \union B', E')$.   \\
		\textbf{Output:} Minimum stable re-allocation of $M$. \\ 
		\begin{enumerate}
			\item $\forall a_i \in A: M'(a_i) \leftarrow M(a_i).$ \\	
			
			\item While $\exists b_j \in B \cup B'$, currently unmatched and $a_i$ in $l(b_j)$ that hasn't been proposed to:\\
				\quad $a_i = $ first member on $l(b_j)$ who $b_j$ hasn't proposed to yet.\\
			    \begin{enumerate}
					\item $b_j$ proposes to $a_i.$ 
					\item If $a_i$ prefers $M'(a_i)$ to $b_j$, do:
						\begin{enumerate}
							\item Reject $b_j$.
						\end{enumerate}

			        \item Else:
						\begin{enumerate}
							\item Unmatch $M'(a_i).$
							\item $M' \leftarrow M' \union (a_i, b_j).$
						\end{enumerate}
			    \end{enumerate}
		    
		    \item Return $M'$.\\
		
            
		\end{enumerate}
	

	\end{wbox}
	\caption{Mechanism $\cM_2$ for adding new B in round $\cR_2$}
	%\label{alg:S1} 
\end{figure} 


\begin{observation}\label{obs:GS-equal}
$\cM_2$ can be thought of as a continuation of Gale-Shapley with the inclusion of new participants, where initially everyone is tentatively matched to their original partners in $M$, and the proposals now come from the side with new participants. 

\end{observation} 

\begin{lemma}\label{sec:new_participant_lemma_2}
If $a_i$ is matched to $b_j$ in any step of $\cM_2$, then $a_i$ is matched to $b_j$ or better in any minimum stable re-allocation.
\end{lemma}

\begin{proof}
The proof is by induction. At the beginning of $\cM_2$ this is true because of Lemma \ref{sec:new_participant_lemma}. Assume during some step $n$, $\cM_2$ matches $a_i$ to $b_j$.
Let $M^*$ be a minimum stable re-allocation where $a_i$ is matched to someone worse than $b_j$. Then $b_j$ must prefer its partner in $M^*$ to $a_i$, but this means that $M^*(b_j)$ must have rejected $b_j's$ proposal in $\cM_2$ and at step $n$, $M^*(b_j)$ was matched to someone better, contradicting the inductive hypothesis.\\

\end{proof}

\begin{theorem} \label{sec:new_participants_theorem}
	$\cM_2$ is a polynomial time mechanism that computes an A-Pessimal minimum stable re-allocation, $M'$, over $M, (A, B \union B', E')$
\end{theorem}

\begin{proof}
	Suppose $a_i \in A$ such that $M(a_i) \neq M'(a_i)$. By Lemma \ref{sec:new_participant_lemma_2} if $a_i$ is not matched to $M'(a_i)$, or better then $(a_i, M'(a_i))$ forms a blocking pair. Since $\cM_2$ only moves $a_i$ from their original partners when they have to be moved, it performs the minimum number of re-allocations.\\
	To see that it is A-Pessimal, let $M^*$ be another minimum stable re-allocation where there is an $a_i$ who prefers $M'(a_i)$ to $M^*(a_i)$. By Lemma $\ref{sec:new_participant_lemma_2}$, $a_i$ must be matched to $M'(a_i)$ or better in any minimum stable re-allocation, a contradiction.\\
\end{proof}


\begin{lemma}
	There exists a mechanism $\cM_3$, that finds an A-optimal minimum stable re-allocation.

\end{lemma}

\begin{proof}
	From Lemma $\ref{sec:decompose-lemma}$, the A-optimal minimum stable re-allocation corresponds to the A-optimal stable matching in $S_{G'}$. To find an A-optimal stable matching of $S_{G'}$, run $M_2$ on the whole instance and find the sets $A_R, B_R, M_F$. We can then construct $G'$, and run Gale-Shapley on this instance to find the A-optimal matching, $M_{opt}$, in $S_{G'}.$ Applying Lemma $\ref{sec:compose-lemma}$, taking the union of $M_F$ and $M_{opt}$ will give an A-optimal minimum stable re-allocation.\\ 

\end{proof}


